FM-Loc: Using Foundation Models for Improved Vision-based Localization

Visual place recognition is essential for vision-based robot localization and SLAM. Despite the tremendous progress made in recent years, place recognition in changing environments remains challenging. A promising approach to cope with appearance variations is to leverage high-level semantic features like objects or place categories. In this paper, we propose FM-Loc which is a novel image-based localization approach based on Foundation Models that uses the Large Language Model GPT-3 in combination with the Visual-Language Model CLIP to construct a semantic image descriptor that is robust to severe changes in scene geometry and camera viewpoint. We deploy CLIP to detect objects in an image, GPT-3 to suggest potential room labels based on the detected objects, and CLIP again to propose the most likely location label. The object labels and the scene label constitute an image descriptor that we use to calculate a similarity score between the query and database images. We validate our approach on real-world data that exhibit significant changes in camera viewpoints and object placement between the database and query trajectories. The experimental results demonstrate that our method is applicable to a wide range of indoor scenarios without the need for training or fine-tuning.

==> sources.tex <==
@string{IROS = "IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS)"}
@string{ICRA = "IEEE International Conference on Robotics and Automation (ICRA)"}

@string{TRO = "IEEE Transactions on Robotics (T-RO)"}
@string{RAL = "IEEE Robotics and Automation Letters (RA-L)"}

@string{RSS = "Robotics: Science and Systems (RSS)"}

@string{IJRR = "International Journal of Robotics Research (IJRR)"}

@string{ECCV = "European Conference on Computer Vision (ECCV)"}
@string{ICCV = "International Conference on Computer Vision (ICCV)"}
@string{CVPR = "Conference on Computer Vision and Pattern Recognition (CVPR)"}

@string{ICML = "International Conference on Machine Learning (ICML)"}


@string{TPAMI = "IEEE Transactions on Pattern Analysis and Machine Intelligence (TPAMI)"}
@string{IJCV = "International Journal of Computer Vision (IJCV)"}

@string{THREEDV = "International Conference on 3D Vision (3DV)"}
@string{ISMAR = "IEEE International Symposium on Mixed and Augmented Reality (ISMAR)"}

@string{SIG7492 = "ACM SIGGRAPH Computer Graphics"}
@string{SIG9301 = "International Conference on Computer Graphics and Interactive Techniques (SIGGRAPH)"}
@string{TOG = "ACM Transactions on Graphics (TOG)"}

@string{NeurIPS = "Advances in Neural Information Processing Systems (NeurIPS)"}

@inproceedings{patchnetvlad,
  title={{Patch-NetVLAD}: Multi-scale fusion of locally-global descriptors for place recognition},
  author={Hausler, Stephen and Garg, Sourav and Xu, Ming and Milford, Michael and Fischer, Tobias},
  booktitle=CVPR,
  year={2021}
}

@article{bommasani2021opportunities,
  title={On the opportunities and risks of foundation models},
  author={Bommasani, Rishi and Hudson, Drew A and Adeli, Ehsan and Altman, Russ and Arora, Simran and von Arx, Sydney and Bernstein, Michael S and Bohg, Jeannette and Bosselut, Antoine and Brunskill, Emma and others},
  journal={arXiv preprint arXiv:2108.07258},
  year={2021}
}

@inproceedings{devlin2018bert,
  title={{BERT}: Pre-training of Deep Bidirectional Transformers for Language Understanding},
  author={Devlin, Jacob and Chang, Ming-Wei and Lee, Kenton and Toutanova, Kristina},
  booktitle={Proceedings of NAACL-HLT},
  year={2019}
}

@inproceedings{brown2020language,
  title={Language models are few-shot learners},
  author={Brown, Tom and Mann, Benjamin and Ryder, Nick and Subbiah, Melanie and Kaplan, Jared D and Dhariwal, Prafulla and Neelakantan, Arvind and Shyam, Pranav and Sastry, Girish and Askell, Amanda and others},
  booktitle=NeurIPS,
  year={2020}
}

@inproceedings{chainofthought,
title={Chain of Thought Prompting Elicits Reasoning in Large Language Models},
author={Jason Wei and Xuezhi Wang and Dale Schuurmans and Maarten Bosma and Brian Ichter and Fei Xia and Ed H. Chi and Quoc V Le and Denny Zhou},
booktitle=NeurIPS,
year={2022}
}

@article{socratic,
  title={Socratic models: Composing zero-shot multimodal reasoning with language},
  author={Zeng, Andy and Wong, Adrian and Welker, Stefan and Choromanski, Krzysztof and Tombari, Federico and Purohit, Aveek and Ryoo, Michael and Sindhwani, Vikas and Lee, Johnny and Vanhoucke, Vincent and others},
  journal={arXiv preprint arXiv:2204.00598},
  year={2022}
}

@inproceedings{CLIP,
  title={Learning transferable visual models from natural language supervision},
  author={Radford, Alec and Kim, Jong Wook and Hallacy, Chris and Ramesh, Aditya and Goh, Gabriel and Agarwal, Sandhini and Sastry, Girish and Askell, Amanda and Mishkin, Pamela and Clark, Jack and others},
  booktitle=ICML,
  year={2021}
}

@inproceedings{cocodataset,
  title={Microsoft coco: Common objects in context},
  author={Lin, Tsung-Yi and Maire, Michael and Belongie, Serge and Hays, James and Perona, Pietro and Ramanan, Deva and Doll{\'a}r, Piotr and Zitnick, C Lawrence},
  booktitle=ECCV,
  year={2014}
}

@inproceedings{shah2022robotic,
  title={Robotic navigation with large pre-trained models of language, vision, and action},
  author={Shah, Dhruv},
  booktitle={NeurIPS 2022 Foundation Models for Decision Making Workshop},
  year={2022}
}

@inproceedings{shah2021ving,
  title={Ving: Learning open-world navigation with visual goals},
  author={Shah, Dhruv and Eysenbach, Benjamin and Kahn, Gregory and Rhinehart, Nicholas and Levine, Sergey},
  booktitle=ICRA,
  year={2021}
}

@article{huang2022visual,
  title={Visual Language Maps for Robot Navigation},
  author={Huang, Chenguang and Mees, Oier and Zeng, Andy and Burgard, Wolfram},
  journal={arXiv preprint arXiv:2210.05714},
  year={2022}
}

@inproceedings{dorbala2022clip,
    title={{CLIP-Nav}: Using {CLIP} for Zero-Shot Vision-and-Language Navigation},
    author={Vishnu Sashank Dorbala and Gunnar A Sigurdsson and Jesse Thomason and Robinson Piramuthu and Gaurav S. Sukhatme},
    booktitle={Workshop on Language and Robotics at CoRL 2022},
    year={2022}
}

@article{gadre2022clip,
  title={{CoWs} on {Pasture}: Baselines and Benchmarks for Language-Driven Zero-Shot Object Navigation},
  author={Gadre, Samir Yitzhak and Wortsman, Mitchell and Ilharco, Gabriel and Schmidt, Ludwig and Song, Shuran},
  journal={arXiv preprint arXiv:2203.10421},
  year={2022}
}

@inproceedings{brohan2022can,
  title={Do as {I} can, not as {I} say: Grounding language in robotic affordances},
  author={Brohan, Anthony and Chebotar, Yevgen and Finn, Chelsea and Hausman, Karol and Herzog, Alexander and Ho, Daniel and Ibarz, Julian and Irpan, Alex and Jang, Eric and Julian, Ryan and others},
  booktitle={Conference on Robot Learning (CoRL)},
  year={2022}
}

@article{chen2022open,
  title={Open-vocabulary queryable scene representations for real world planning},
  author={Chen, Boyuan and Xia, Fei and Ichter, Brian and Rao, Kanishka and Gopalakrishnan, Keerthana and Ryoo, Michael S and Stone, Austin and Kappler, Daniel},
  journal={arXiv preprint arXiv:2209.09874},
  year={2022}
}

@article{chen2019scene,
  title={Scene classification in indoor environments for robots using context based word embeddings},
  author={Chen, Bao Xin and Sahdev, Raghavender and Wu, Dekun and Zhao, Xing and Papagelis, Manos and Tsotsos, John K},
  journal={arXiv preprint arXiv:1908.06422},
  year={2019}
}

@article{heikel2022indoor,
  title={Indoor Scene Recognition via Object Detection and {TF-IDF}},
  author={Heikel, Edvard and Espinosa-Leal, Leonardo},
  journal={Journal of Imaging},
  volume={8},
  number={8},
  pages={209},
  year={2022}
}

@inproceedings{redmon2016you,
  title={You only look once: Unified, real-time object detection},
  author={Redmon, Joseph and Divvala, Santosh and Girshick, Ross and Farhadi, Ali},
  booktitle=CVPR,
  year={2016}
}

@ARTICLE{vysotska2016lazy,
  author={Vysotska, Olga and Stachniss, Cyrill},
  journal=RAL, 
  title={Lazy Data Association For Image Sequences Matching Under Substantial Appearance Changes}, 
  year={2016},
  volume={1},
  number={1},
  pages={213-220}
}

@INPROCEEDINGS{vysotska2015efficient,
  author={Vysotska, Olga and Naseer, Tayyab and Spinello, Luciano and Burgard, Wolfram and Stachniss, Cyrill},
  booktitle=ICRA,
  title={Efficient and effective matching of image sequences under substantial appearance changes exploiting {GPS} priors}, 
  year={2015}
}

@inproceedings{vysotska2017relocalization,
	title     = {Relocalization under Substantial Appearance Changes using Hashing},
	author    = {O. Vysotska and C. Stachniss},
	booktitle = {9th Workshop on Planning, Perception and Navigation for Intelligent Vehicles at the IEEE},
	year      = {2017}
}

@inproceedings{arandjelovic2016netvlad,
  title={{NetVLAD}: {CNN} architecture for weakly supervised place recognition},
  author={Arandjelovic, Relja and Gronat, Petr and Torii, Akihiko and Pajdla, Tomas and Sivic, Josef},
  booktitle=CVPR,
  year={2016}
}

@article{tomitua2021convsequential,
  title={{ConvSequential-SLAM}: A sequence-based, training-less visual place recognition technique for changing environments},
  author={Tomit{\u{a}}, Mihnea-Alexandru and Zaffar, Mubariz and Milford, Michael J and McDonald-Maier, Klaus D and Ehsan, Shoaib},
  journal={IEEE Access},
  volume={9},
  pages={118673--118683},
  year={2021}
}


@article{garg2022semantic,
  title={Semantic--geometric visual place recognition: a new perspective for reconciling opposing views},
  author={Garg, Sourav and Suenderhauf, Niko and Milford, Michael},
  journal=IJRR,
  volume={41},
  number={6},
  pages={573--598},
  year={2022}
}

@inproceedings{yu2018ds,
  title={{DS-SLAM}: A semantic visual {SLAM} towards dynamic environments},
  author={Yu, Chao and Liu, Zuxin and Liu, Xin-Jun and Xie, Fugui and Yang, Yi and Wei, Qi and Fei, Qiao},
  booktitle=IROS,
  year={2018}
}

@inproceedings{bowman2017probabilistic,
  title={Probabilistic data association for semantic {SLAM}},
  author={Bowman, Sean L and Atanasov, Nikolay and Daniilidis, Kostas and Pappas, George J},
  booktitle=ICRA,
  year={2017}
}

@article{gomez2020object,
  title={Object-based pose graph for dynamic indoor environments},
  author={Gomez, Clara and Hernandez, Alejandra C and Derner, Erik and Barber, Ramon and Babu{\v{s}}ka, Robert},
  journal=RAL,
  volume={5},
  number={4},
  pages={5401--5408},
  year={2020}
}
